BlenderGym: Benchmarking Foundational Model Systems for Graphics Editing

3D graphics editing is crucial in applications like movie production and game design, yet it remains a time-consuming process that demands highly specialized domain expertise. Automating this process is challenging because graphical editing requires performing a variety of tasks, each requiring distinct skill sets. Recently, vision-language models (VLMs) have emerged as a powerful framework for automating the editing process, but their development and evaluation are bottlenecked by the lack of a comprehensive benchmark that requires human-level perception and presents real-world editing complexity. In this work, we present BlenderGym, the first comprehensive VLM system benchmark for 3D graphics editing. BlenderGym evaluates VLM systems through code-based 3D reconstruction tasks. We evaluate closed- and open-source VLM systems and observe that even the state-of-the-art VLM system struggles with tasks relatively easy for human Blender users. Enabled by BlenderGym, we study how inference scaling techniques impact VLM's performance on graphics editing tasks. Notably, our findings reveal that the verifier used to guide the scaling of generation can itself be improved through inference scaling, complementing recent insights on inference scaling of LLM generation in coding and math tasks. We further show that inference compute is not uniformly effective and can be optimized by strategically distributing it between generation and verification.

==> figures/alignment_2.tex <==

\begin{wrapfigure}{r}{0.26\textwidth}
\vspace{-1.5em} 
%\vspace{1em} 
\hspace{-1em} 
\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/verifier_alignment_cut.jpg}
\label{fig:alignment_2}  
\vspace{-1em} 
\end{wrapfigure}


% \begin{figure}{t}
% \centering
% \vspace{-1em} 
% \hspace{-1.8em}
% \includegraphics[width=.5\linewidth, trim=0 0 0 0, clip]{images/verifier_alignment_cut.jpg}
% %\caption{VLM-human verifier alignment rate with ``equal'' choice disabled.}
% \label{fig:alignment_2}  
% \vspace{-1em} 
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \vspace{-1em} 
%     \hspace{-1.8em}
%     \includegraphics[width=0.48\linewidth, trim=0 0 0 0, clip]{images/verifier_alignment_cut.jpg}
%     % \caption{VLM-human verifier alignment rate with ``equal'' choice disabled.}
%     \label{fig:alignment_2}  
%     \vspace{-1em} 
% \end{figure}



==> figures/borrow.tex <==
\setlength{\intextsep}{0pt}
\setlength{\columnsep}{10pt}
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{images/borrow.pdf}
\caption{Examples of scenes, objects, and procedural materials based on BlenderAlchemy, Blenderkit, and Infinigen.}
\label{fig: borrow}
\end{figure}



==> figures/comprehensive.tex <==
\setlength{\intextsep}{0pt}
\setlength{\columnsep}{10pt}
\begin{figure}
\centering
\vspace{-140pt}
\includegraphics[width=\linewidth, page=4]{images/supp_views.pdf}
\vspace{-100pt}
\caption{Examples of ``comprehensive'' camera views.}
\label{fig: comprehensive_views}
\vspace{-10pt}
\end{figure}



==> figures/full_benchmark_exmps.tex <==
\begin{figure*}[t]
\begin{center}
    %\hspace{0cm} Translation \hspace{3cm} Rotation\\
\includegraphics[width=\linewidth]{images/exp_scenes.png}
\end{center}
\vspace{-1em}
    
    \caption{\TODO{swap out images}Example source-target pairs for all five tasks: materials, geonodes, lighting, placement, and shapekey.
    }
    \vspace{-1em}
    \label{fig:exmpl_scenes}
\end{figure*}


==> figures/merged.tex <==

\begin{figure}[h]
    \centering
    \vspace{-1em} 
    \includegraphics[width=0.9\linewidth, trim=0 0 0 0, clip]{images/merged.jpg}
    % \caption{VLM-human verifier alignment rate with ``equal'' choice disabled.}
    \label{fig:alignment_2}  
    \vspace{-2.5em} 
\end{figure}


==> figures/multi_facet_comp.tex <==
\begin{figure}[t]
\centering
    %\hspace{0cm} Translation \hspace{3cm} Rotation\\
    \includegraphics[width=\linewidth]{images/radar.png}
    \vspace{-2em}
    \caption{\TODO{multi facet comparison for different tasks}
    }
    \vspace{-1em}
    \label{fig:multi_comp}
\end{figure}


==> figures/scaling_res.tex <==
\begin{figure*}[ht]
\centering
\vspace{1em}
\includegraphics[width=\linewidth, height=150px]{images/placeholder.pdf}
\vspace{-2em}
\caption{\TODO{table comparison for inference scaling}
}
\label{fig:quali_3d}
\end{figure*}

==> figures/trend_imitation.tex <==
\begin{wrapfigure}{r}{0.3\textwidth}
\centering
\vspace{-1.3em}
\hspace{-2em}
 % Move the figure left
\includegraphics[width=\linewidth, trim=0 10 0 0, clip]{images/placement.png}
% \caption{}
\label{fig:alignment_2} 
\vspace{-1em} 
\end{wrapfigure}


==> tables/alignment.tex <==
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
Verifier & Claude3.5Sonnet & GPT4o & GPT4Turbo & Gemini1.5Flash & Human \\
\midrule
Alignment    &  77.0\%  & 67.6\% & 75.4\%   & 72.3\% & 88.5\% \\
\bottomrule
\end{tabular}%
}
\caption{Alignment rate of VLMs with human verifier, and human verifier within themselves.}
\label{tab: alignment}
\end{table}




==> tables/llama.tex <==
\begin{table}[h]
\label{tab: alignment}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
VLM & Qwen & MiniCPM & Intern & Phi \\
\midrule
Average Percentage Increase    &  77.0\%  & 67.6\% & 75.4\%   & 72.3\% & 88.5\% \\
\bottomrule
\end{tabular}%
}
\caption{Average percentage increase of open-source VLMs after applying Llama3.1-8b\cite{} as code editor.}
\end{table}

==> tables/main_table_average.tex <==
\begin{table*}[ht]
\centering
%\renewcommand{\arraystretch}{1.5} % Adjust row height
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Shapekey} & \multicolumn{3}{c}{Placement} & \multicolumn{3}{c}{Geometry Nodes} & \multicolumn{2}{c}{Lighting $(\times10^{-2})$} & \multicolumn{2}{c}{Material} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
Model & N-CLIP $\downarrow$ $(\times10^{-3})$ & PL $\downarrow$ $(\times10^{-3})$ & CD $\downarrow$ & N-CLIP $\downarrow$ & PL $\downarrow$ & CD $\downarrow$ & N-CLIP $\downarrow$ & PL $\downarrow$ & CD $\downarrow$ & N-CLIP $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & PL $\downarrow$ \\ \hline
gpt-4-turbo & 22.23& 6.675& 1.055& 12.66  & 3.968 & 13.86   &  &  &  & 4.331 & 3.173 &  &  \\ 
gpt-4o & 20.60 & 6.235 & 1.033 &  11.46 & 2.197 & 11.12  &  &  &  & \underline{4.100} & 3.298 &  &  \\ 
ClaudeV & 26.17 & 8.588 & 1.236 &  11.48 & 1.802 & 15.52  &  &  &  & 4.756 & 3.637 &  &  \\ 
ClaudeS & 20.95 & 6.158 & 0.9919&  10.95 & 2.333 & 13.84  &  &  &  & \textbf{3.940} & \underline{3.021} &  &  \\ 
GeminiV & \underline{12.46 }& \underline{4.471} & 1.208&  &  &  &  &  &  & 4.611 & 3.885 &  &  \\ 
Qwen & \textbf{10.09} & \textbf{2.432} & \textbf{0.331} &  &  &  &  &  &  & \textit{4.217} & 3.717 &  &  \\ 
Qwen-Llama & \textit{19.55} & 5.656 & 0.895 &  &  &  &  &  &  & 5.044 & 3.734 &  &  \\ 
Phi & 20.07 & \textit{5.153} & \textit{0.707} &  &  &  &  &  &  & 5.235 & 3.586 &  &  \\ 
Phi-Llama & 22.88 & 6.725 & 1.036 &  &  &  &  &  &  & 5.509 & 3.872 &  &  \\ 
MiniCPM & 25.70 & 7.793 & 1.131 &  &  &  &  &  &  & 5.215 & \textbf{2.924} &  &  \\ 
MiniCPM-Llama & 23.95 & 6.964 & 1.041 &  &  &  &  &  &  & 5.491 & 3.212 &  &  \\ 
Intern & 25.20 & 7.935 & 1.167 &  &  &  &  &  &  & 5.444 & \textit{3.086} &  &  \\ 
Intern-Llama & 24.75 & 7.166 & 1.019 &  &  &  &  &  &  & 5.787 & 3.512 &  &  \\ \hline
\end{tabular}
}
\caption{Metric Scores of Average Edits}
\end{table*}


==> tables/main_table_best.tex <==
\begin{table*}[ht]
\centering
%\renewcommand{\arraystretch}{1.5} % Adjust row height
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Shapekey $(\times10^{-3})$} & \multicolumn{3}{c}{Placement} & \multicolumn{3}{c}{Geometry Nodes} & \multicolumn{2}{c}{Lighting $(\times10^{-2})$} & \multicolumn{2}{c}{Material} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
Model & PL $\downarrow$ & N-CLIP $\downarrow$ & CD $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & CD $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & CD $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ \\ \hline
GPT4T & 3.512& 12.76& 0.762&  3.599& 9.447& 6.942&  &  &  & \textbf{1.300} & 2.461&  &  \\ 
GPT4o & 3.401& 11.52& 0.776&  4.518& 9.163& 9.529&  &  &  & 1.879 & 2.588&  &  \\ 
ClaudeV & 4.568& 15.34& 0.996 &  4.660& 9.530& 9.331&  &  &  & 1.954 & 2.953&  &  \\ 
ClaudeS & 2.827& 10.01& 0.731 &  3.349& 7.346& 6.776&  &  &  & \underline{1.360} & 2.606&  &  \\ 
GeminiV & 7.021& 22.40& 1.165&  4.971& 11.16& 9.047&  &  &  & 2.540& 4.873&  &  \\ 
Qwen & 6.508& 22.82& 1.085&  9.854& 23.15& 9.334&  &  &  & 2.407& 4.470&  &  \\ 
Qwen-Llama & 3.070& 12.45& 0.829&  4.195&  15.10&  5.286&  &  &  & 2.220 & 4.183&  &  \\ 
Phi & 4.670& 16.43& 0.762& & &  &  &  &  & 2.446 & 4.034&  &  \\ 
Phi-Llama & 4.333& 14.96& 0.809&  6.039&  20.19&  5.358&  &  &  & 2.953& 4.121&  &  \\ 
MiniCPM & 4.596& 16.73& 0.939& 7.040& 22.81&  8.304&  &  &  & 1.791& 4.068&  &  \\ 
MiniCPM-Llama & 2.377& 9.700& 0.966&  2.739&  5.526&  2.702&  &  &  & 1.875& 3.356&  &  \\ 
Intern & 3.855& 14.78& 0.701 &  10.06&  28.28&  8.718&  &  &  & 1.762& 3.872&  &  \\ 
Intern-Llama & 2.874 & 1.078 & 0.658&  4.067&  11.67&  2.425&  &  &  & 1.792 & 3.264&  &  \\ \hline
\end{tabular}
}
\caption{Metric Scores of Best Edits}
\label{tab:best table}
\end{table*}



==> tables/metrics_alignment.tex <==
% \begin{nolinenumbers} % Disable line numbers for wrapped content
% \begin{wraptable}{r}{0.3\textwidth}
% % \vspace{-0.8em}
% \centering
% \footnotesize
% \scriptsize % Use smaller font size
% \setlength{\tabcolsep}{1pt} % Reduce column padding
% \begin{tabular}{@{}cccc@{}} % Adjusted column layout
% \toprule
% Metrics & N-CLIP & PL & CD \\
% \midrule
% Alignment & 86.0\% & 88.9\% & 91.4\% \\
% \bottomrule
% \end{tabular}
% \label{tab: metrics_alignment}
% %\vspace{1em}
% \end{wraptable}
% \end{nolinenumbers} % Re-enable line numbers

\begin{wraptable}{r}{0.2\textwidth} % Slightly increase width to avoid overfull issue
%\vspace{-0.8em}
\centering
\footnotesize
\scriptsize % Use smaller font size
\setlength{\tabcolsep}{1pt} % Reduce column padding
\begin{tabular}{@{}cccc@{}} % Adjusted column layout
\toprule
Metrics & N-CLIP & PL & CD \\
\midrule
Alignment & 86.0\% & 88.9\% & 91.4\% \\
\bottomrule
\end{tabular}
\label{tab: metrics_alignment}
%\vspace{1em}
\end{wraptable}

% \begin{table}[t]
% \vspace{-2em}
% \centering
% \hspace{-2em}
% \footnotesize
% \caption{Alignment rate}
% \scriptsize % Use smaller font size
% \setlength{\tabcolsep}{1pt} % Reduce column padding
% \begin{tabular}{@{}cccc@{}} % Adjusted column layout
% \toprule
% Metrics & N-CLIP & PL & CD \\
% \midrule
% Alignment & 86.0\% & 88.9\% & 91.4\% \\
% \bottomrule
% \end{tabular}
% \label{tab: metrics_alignment}
% \vspace{-2em}
% \end{table}

% \begin{table}[t]
%     \hspace{3em} % Moves table slightly to the right
%     \vspace{1em}
%     \centering
%     \footnotesize
%     \caption{Alignment rate}
%     \scriptsize % Use smaller font size
%     \setlength{\tabcolsep}{2pt} % Reduce column padding
%     \begin{tabular}{@{}cccc@{}} % Adjusted column layout
%         \toprule
%         Metrics & N-CLIP & PL & CD \\
%         \midrule
%         Alignment & 86.0\% & 88.9\% & 91.4\% \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:metrics_alignment}
%     \vspace{-2em}
% \end{table}


==> tables/pseudocode_1.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{\linewidth}|}
\hline
\textbf{Algorithm 1: Scaled Verification} \\
\hline
\textbf{Function} ScaledSelect(List of proposal candidates $\{S_1, S_2, .., S_n\}$, Verifier $V$, Reselection parameter $k$): \\
\hspace{2em}Initialize \textit{winner\_list} as an empty list. \\
\hspace{2em}\textbf{for} $i = 1$ to $k$ \textbf{do} \\
\hspace{4em} $\{S_1', S_2', \dots, S_n'\} \gets \text{shuffle} (\{S_1, S_2, .., S_n\})$\\
\hspace{4em} $winner \gets \text{SingleSelection}(\{S_1', S_2', \dots, S_n'\}, V)$ \\
\hspace{4em} Append $winner$ to \textit{winner\_list}. \\
\hspace{2em}\textbf{end for} \\
\hspace{2em}$final\_winner \gets \text{single\_selection}(\text{winner\_list}, V)$ \\
\hspace{2em}\textbf{return} $final\_winner$ \\
\hline
\end{tabular}
\end{table}


==> tables/scaling_table.tex <==
\begin{table*}[ht]
\centering
%\renewcommand{\arraystretch}{1.5} % Adjust row height
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Shapekey(1-16)}} & \multicolumn{3}{c}{\textbf{Placement(1-16)}} & \multicolumn{2}{c}{\textbf{Lighting(1-16)}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-9} 
\multicolumn{1}{c}{\textbf{Model}} & PL& N-CLIP & CD& PL & N-CLIP & CD & PL & N-CLIP \\ \hline
Qwen(2x3) &  &  &  &  &  &  &  &  \\ 
Qwen(3x4) &  &  &  &  &  &  &  &  \\ 
Qwen(4x8) &  &  &  &  &  &  &  &  \\ 
Qwen(8x16) &  &  &  &  &  &  &  &  \\
Qwen(16x32) &  &  &  &  &  &  &  &  \\ 
Qwen(32x32) &  &  &  &  &  &  &  &  \\ 
GPT-4-Turbo &  &  &  &  &  &  &  &  \\ 
GPT-4o &  &  &  &  &  &  &  &  \\ 
Claude-3-Haiku &  &  &  &  &  &  &  &  \\ 
Claude-3.5-Sonnet &  &  &  &  &  &  &  &  \\ 
GeminiV &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
%}
\caption{Comprehensive Table of Models and Metrics}
\end{table*}

==> tables/structure.tex <==
% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{3pt} 

% \scriptsize
% \begin{tabular}{@{}lccccccccccccc@{}}

% \toprule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Blend Shape} & \multicolumn{3}{c}{Placement} & \multicolumn{3}{c}{Geometry} & \multicolumn{2}{c}{Lighting} & \multicolumn{2}{c}{Material} \\ 
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
% Model & PL $\downarrow$ & N-CLIP $\downarrow$ & CD $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & CD $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & CD $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ & PL $\downarrow$ & N-CLIP $\downarrow$ \\ \midrule

% BlenderGPT-gpt4o & 9.747 & 26.73 & 1.157 & 12.85& 35.10&  9.667&  3.567&  15.87&  0.731& 3.293 & 5.112 &  2.546&  13.84\\ 
% BlenderGPT-claude-3.5-sonnet & 8.372 & 20.74 & 1.063 & 12.11 & 35.45&  14.93&  3.567&  11.44&  0.731 & 3.700 & 4.300 &  2.699&  12.92\\
% % BlenderGPT-gemini-1.5-flash & 10.87 & 29.30 & 1.243 & 13.97& 37.59&  12.04&  3.567&  11.44&  0.731& 3.673 & 5.914 &  2.722&  13.47\\


% % Chain-gemini-1.5-flash & 7.354 & 24.54& 1.036 & 16.14& 35.55&  9.667&  3.567&  11.44&  0.731& 3.810 & 6.467 &  --&  --\\
% \midrule
% % \textbf{Human}& \textbf{0.934}& \textbf{9.12}& \textbf{0.399}& \textbf{0.423}& \textbf{13.34} & \textbf{1.532} & \textbf{1.269} & \textbf{2.434} & \textbf{0.334} & \textbf{1.239} & \textbf{2.932} & \textbf{0.629} & \textbf{3.043}  \\

% \bottomrule
% \end{tabular}

% \label{tab: other_model_table}
% \end{table*}
\vspace{-.8em}
\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt} 
\scriptsize
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{Blend Shape} & \multicolumn{1}{c}{Placement} & \multicolumn{1}{c}{Geometry} & \multicolumn{1}{c}{Lighting} & \multicolumn{1}{c}{Material} \\ \midrule

BlenderGPT-GPT4o & 9.747 & 12.85 & 3.223 & 3.293 & 2.546 \\ 
BlenderGPT-ClaudeS & 8.372 & 12.11 & 3.167 & 3.786 & 2.699 \\
\textbf{Human(10 users)} & \textbf{1.432} & \textbf{0.812} & \textbf{1.228} & \textbf{0.965} & \textbf{0.347} \\
\bottomrule
\end{tabular}
\vspace{-1.2em}
\caption{Performance of other pipelines and scaled human editor.}
\label{tab: other_model_table}
\vspace{-3.8em}
\end{table}






==> tables/trend_table.tex <==
% \begin{table}[h]
% \centering
% \scriptsize
% \vspace{-1em}
% \setlength{\tabcolsep}{2pt} 
% \renewcommand{\arraystretch}{0.9}
% \begin{tabular}{@{}lcccccccc@{}} 
% \toprule
% & \multicolumn{4}{c}{Placement (PL$\downarrow$)} & \multicolumn{4}{c}{Geometry (CD$\downarrow$)} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
% Goal Input & GPT4o & MiniCPM & ClaudeS & Gemini & GPT4o & ClaudeS & MiniCPM & Gemini \\ \midrule
% Image & 10.95 & 11.19 & 11.39 & 12.28 & 0.511 & 0.652 & 0.694 & 0.744 \\ 
% Text & 14.88 & 15.51 & 15.96 & 16.96 & 0.560 & 0.666 & 0.844 & 0.980  \\
% \bottomrule
% \end{tabular}
% \vspace{-1.2em}
% \label{tab:trend}
% \end{table}

\begin{table}[h]

\centering
\scriptsize
\vspace{-1em}
\setlength{\tabcolsep}{2pt} 
\renewcommand{\arraystretch}{0.9}
\resizebox{\linewidth}{!}{
% % Add an arrow above the table
% \begin{tikzpicture}
% \node at (4.5,.2) {\textbf{Better Performance}};
% \draw[<-,thick] (.5,0) -- (9,0);
% \end{tikzpicture}

%\vspace{0.5em} % Adjust space between arrow and table

% \begin{tabular}{@{}lcccccccc@{}} 
% \toprule
% & \multicolumn{4}{c}{Placement (PL$\downarrow$)} & \multicolumn{4}{c}{Geometry (CD$\downarrow$)} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
% Goal Format & GPT4o & MiniCPM & ClaudeS & Gemini & GPT4o & ClaudeS & MiniCPM & Gemini \\ \midrule
% Image & 10.95 & 11.19 & 11.39 & 12.28 & 0.511 & 0.652 & 0.694 & 0.744 \\ 
% Text & 14.88 & 15.51 & 15.96 & 16.96 & 0.560 & 0.666 & 0.844 & 0.980  \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.2em}
% % \caption{Performance of other pipelines and scaled human editor.}
% \vspace{-3.2em}
% \label{tab:trend}
% \end{table}

\begin{tabular}{@{}lcccccccc@{}} 
\toprule
& \multicolumn{4}{c}{Placement (PL$\downarrow$)} & \multicolumn{4}{c}{Geometry (CD$\downarrow$)} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
Goal Format & MiniCPM & Gemini & GPT4o & ClaudeS & GPT4o & ClaudeS & MiniCPM & Gemini \\ \midrule
Image & 9.637 & 10.58 & 10.95 & 11.39 & 0.511 & 0.652 & 0.694 & 0.744 \\ 
Text & 14.88 & 15.51 & 15.96 & 16.96 & 0.560 & 0.666 & 0.844 & 0.980  \\
\bottomrule
\end{tabular}
}
% \vspace{-1.2em}
% \caption{Performance of other pipelines and scaled human editor.}
\vspace{-3.2em}
\label{tab:trend}
\end{table}


